Formal verification in Solidity and Move: insights from a comparative analysis

Formal verification plays a crucial role in making smart contracts safer, being able to find bugs or to guarantee their absence, as well as checking whether the business logic is correctly implemented. For Solidity, even though there already exist several mature verification tools, the semantical quirks of the language can make verification quite hard in practice. Move, on the other hand, has been designed with security and verification in mind, and it has been accompanied since its early stages by a formal verification tool, the Move Prover. In this paper, we investigate through a comparative analysis: 1) how the different designs of the two contract languages impact verification, and 2) what is the state-of-the-art of verification tools for the two languages, and how do they compare on three paradigmatic use cases. Our investigation is supported by an open dataset of verification tasks performed in Certora and in the Aptos Move Prover.

==> benchmark.tex <==
\endinput

\section{Use cases}
\label{sec:benchmark}

We describe here the use cases considered in our analysis.
%, mentioning the main properties used for our comparison.
The full implementation of the use cases in Solidity and Move, and of all the sets of specifications in CVL and MSL, are in \githuburl.
\enriconote{Evidenziare le caratteristiche particolari di ogni singolo contratto e perché lo rendono interessante a livello di verifica}


%\begin{itemize}
%    \item Bank: mappe, special users (quantificatori?)
%    \item Vault: state-based, tempo, adversary, transaction-ordering dependencies
%    \item Price-bet: external call ($\implies$ aleatorietà, "non-determinismo"), transaction-ordering dependencies (con le tx dell'oracolo) 
%\end{itemize}

\subsection{Bank}

The \contracturl{bank} contract stores assets (native crypto-currency) deposited by users, and pays them out when required. The contract state consists of:
\code{credits}, a key-value map that associates each user with the amount of assets available for that user;
\code{owner}, the address that deploys the contract;
\code{opLimit}, a limit set during contract deployment that restricts the maximum amount that can be deposited or withdrawn in a single transaction. This limit applies to all users except the owner.
The contract has the following entry points:
\begin{itemize}
\item \code{deposit}, which allows anyone to deposit assets. When a deposit is made, the corresponding amount is added to the credit of the transaction sender.
\item \code{withdraw}, which allows the sender to receive any desired amount of assets deposited in their account. The contract checks that the user has sufficient credit and then transfers the specified amount to the sender.
\end{itemize}
%
We have identified \nBankProperties relevant properties of the Bank contract. 
%For the purpose of the comparison in~\Cref{sec:comparison}, we mention:  \enriconote{check questi elenchi non credo siano aggiornati}
%\enriconote{Togliere? alla fine il testo lo riportiamo già in Sec 4}
%\begin{itemize}
 %   \item \specurl{bank}{credits-leq-balance}: the assets controlled by the contract are (at least) equal to the sum of all the credits.
    
  %  \item \specurl{bank}{deposit-assets-transfer}:     after a successful \code{deposit(amount)}, exactly amount token units pass from the control of the sender to that of the contract.
    % \bartnote{(implica bank/deposit-assets-credit)}
    
    %\item \specurl{bank}{withdraw-not-revert}: a transaction \code{withdraw(amount)} does not abort if \code{amount} is less or equal to the transaction sender's credit and operation limit.
    
    %\item \specurl{bank}{deposit-additivity}: two consecutive successful deposits of $n_1$ and $n_2$ token units performed by the same sender are equivalent to a single deposit of $n_1+n_2$ token units, if $n_1+n_2$ is less than or equal to the sender’s operation limit
%\end{itemize}


\subsection{Vault}

The \contracturl{vault} contract is a security mechanism to prevent an adversary who has stolen the owner's private key from stealing the owner's tokens.
To create the vault, the owner specifies:
itself as the vault's owner;
a recovery key, which can be used to cancel a withdraw request;
a wait time, which has to elapse between a withdraw request and the actual finalization of the cryptocurrency transfer.
The contract has the following entry points:
\begin{itemize}

\item \code{receive(amount)}, which allows anyone to deposit tokens into the contract;

\item \code{withdraw(receiver, amount)}, which allows the owner to issue a withdraw request, specifying the receiver and the desired amount;

\item \code{finalize()}, which allows the owner to finalize the pending withdraw after the wait time has passed since the request;

\item \code{cancel()}, which allows the owner of the recovery key to cancel the withdraw request during the wait time.
\end{itemize}
%
We have identified \nVaultProperties relevant properties of the Vault contract. 

%\noindent
%Among the \nVaultProperties properties we have identified, for the purpose of our comparison, we mention: 
%\begin{itemize}
%    \item \specurl{vault}{keys-immutable}: 
    
%    \item \specurl{vault}{withdraw-withdraw-revert}: a transaction \code{withdraw()} aborts if performed immediately after another \code{withdraw()}	
    
%    \item \specurl{vault}{owner-immutable}: the vault owner never changes.
    
%\end{itemize}


\subsection{Price Bet}

The \contracturl{price-bet} contract allows a single player to place a bet against the contract owner. The bet is based on a future exchange rate between two tokens.
To create the contract, the owner specifies:
itself as the contract owner;
the initial pot, which is transferred from the owner to the contract;
an oracle, \ie a contract that is queried for the exchange rate between two given tokens;
a deadline, \ie a time limit after which the player loses the bet;
a target exchange rate, which must be reached in order for the player to win the bet.
The contract has the following entry points:
\begin{itemize}
\item \code{join()}, which allows a player to join the bet. This requires the player to deposit an amount of native cryptocurrency equal to the initial pot;
\item \code{win()}, which allows the joined player to withdraw the whole contract balance if the oracle exchange rate is greater than the bet rate. The player can call win() multiple times before the deadline. This action is disabled after the deadline;
\item \code{timeout()}, which can be called by anyone after the deadline, and transfers the whole contract balance to the owner
\end{itemize}
%
We have identified \nPricebetProperties relevant properties of the Price Bet contract. 

%\noindent
%Among the \nPricebetProperties properties we have identified, for the purpose of our comparison, we mention: 
%\begin{itemize}
%    \item \specurl{price-bet}{no-frozen-funds}: after the deadline, any user can perform some transaction that transfers the contract pot to the owner
%\end{itemize}


==> properties.tex <==


\endinput
\section{Expressing properties in Certora and Move Prover}
\label{sec:properties}

We report here the code of some of the classes of specifications discussed in ~\Cref{sec:comparison:prover}. Due to the appendix space constraint, we refer to our \href{\githubaddress}{dataset} for a more comprehensive set of examples. The list of properties for each property type can be found  in the associated \href{\sheeturl}{sheet}.

\subsection{Function specs}
 

The  \Cref{fig:specCVL} and \Cref{fig:specMSL} presented in \Cref{sec:background:provers} are examples of function specs.
%Other examples are \enriconote{lista di qualche nome di prop specificata come function spec}






\subsection{State invariants}
\label{sec:appendix:stateInv}

As an example of state invariant, consider the property of \contracturl{vault} that ``\emph{the owner and the recovery key are distinct}'' (\specurl{vault}{keys-distinct}).
Note that, as observed in the \emph{Access control and ownership} paragraph in \Cref{sec:comparison:language}, the \emph{owner} in Move is the address that owns the  resource, while in Solidity it is the a field of the contract. 
An alternative way to specify certain invariants in MSL is through \emph{struct invariant} (\eg \specurl{vault}{state-idle-req-inter}).


 \begin{lstlisting}[language=cvl,caption={Specification of \specurl{vault}{keys-distinct} in CVL}]
invariant keys_distinct()
    currentContract.owner != currentContract.recovery;
\end{lstlisting}


\begin{lstlisting}[language=move,caption={Specification of \specurl{vault}{keys-distinct} in MSL}]
spec vault_addr::vault {
  spec module { 
      use aptos_framework::aptos_coin::{AptosCoin};
      invariant forall a : address where exists<Vault<AptosCoin>>(a):
      		global<Vault<AptosCoin>>(a).recovery != a;
  }
}
\end{lstlisting}

\begin{lstlisting}[language=move,caption={Specification of \specurl{vault}{state-idle-req-inter} in MSL}]
spec vault_addr::vault {
   spec Vault {     invariant (state == IDLE) || (state == REQ);  }
 }
\end{lstlisting}




\subsection{Single-transition invariants}
\label{sec:appendix:singleTransInv}

As an example of single transition invariant, consider the property of \contracturl{bank} that ``\emph{if the assets of a user A are decreased after a transaction (of the Bank contract), then that transaction must be a deposit where A is the sender}'' (\specurl{bank}{assets-dec-onlyif-deposit}).
As  observed in the \emph{Single-transition invariants} paragraph in \Cref{sec:comparison:prover}, in MSL the property can only be verified through the contrapositive 
(\ie, ``\emph{for every transaction that is not a \code{deposit()}, or for which A is
not the sender, then the assets of A are not decreased}''), 
using a set of function specs. 
Note that, in the case \contracturl{bank} had a higher number of functions, the size of the MSL specification would grow proportionally, while the CVL spec size would remain constant.


\begin{lstlisting}[language=cvl,caption={Specification of \specurl{bank}{assets-dec-onlyif-deposit} in CVL}]

rule assets_dec_onlyif_deposit {
  env e; method f; calldataarg args; address a;
  require e.msg.sender != currentContract;
  require a != e.msg.sender;
  require a != currentContract; // check that sender is not the contract 
    
  mathint old_a_balance = nativeBalances[a];
  f(e, args);
  mathint new_a_balance = nativeBalances[a];

  assert new_a_balance < old_a_balance => (f.selector == sig:deposit().selector && e.msg.sender == a);
}
\end{lstlisting}


\begin{lstlisting}[language=move,caption={Specification of \specurl{bank}{assets-dec-onlyif-deposit} in MSL}]

spec bank_addr::bank {
  use std::features;    
  spec withdraw {
    let sender_coins_value = global<coin::CoinStore<AptosCoin>>(signer::address_of(sender)).coin.value;
    let post sender_coins_value_post = global<coin::CoinStore<AptosCoin>>(signer::address_of(sender)).coin.value;
    requires !features::spec_is_enabled(features::COIN_TO_FUNGIBLE_ASSET_MIGRATION);
    ensures sender_coins_value_post >= sender_coins_value;
  }
  spec deposit {
    let addr_sender = signer::address_of(sender);
    let bank_credits = global<Bank>(owner).credits;
    let post bank_credits_post = global<Bank>(owner).credits;
    ensures forall a: address where a!=addr_sender : 
      global<coin::CoinStore<AptosCoin>>(a).coin.value 
      >= old(global<coin::CoinStore<AptosCoin>>(a).coin.value);
  }
}
\end{lstlisting}





%\bartnote{forse non riusciamo a mettere un esempio di tutto: farei solo function spec e invariants}

%\enriconote{function spec nel Background, metterei State invariants e single transition, e per le altre link a qualche spec del dataset? (o versione estesa arxiv?)}

\subsection{Multiple-transition invariants}

An example of multiple-transition invariant is \specurl{vault}{finalize-or-cancel-twice-revert}, only expressible in CVL.\footnote{\url{\githubaddress/blob/main/contracts/vault/certora/finalize-or-cancel-twice-revert.spec}}

\subsection{Metamorphic properties}
An example of metamorphic property is \specurl{bank}{withdraw-additivity}, only expressible in CVL.\footnote{\url{\githubaddress/blob/main/contracts/bank/certora/withdraw-additivity.spec}}




\begin{lstlisting}[language=cvl,caption={Specification of \specurl{bank}{deposit-assets-transfer} in CVL}]
rule deposit_assets_transfer {
  env e;
  require e.msg.sender != currentContract;
  mathint old_contract_balance = nativeBalances[currentContract];
  mathint old_sender_balance = nativeBalances[e.msg.sender];
  deposit(e);
  mathint new_contract_balance = nativeBalances[currentContract];
  assert new_contract_balance == old_contract_balance + e.msg.value;
  assert nativeBalances[e.msg.sender] == old_sender_balance - e.msg.value;
}
\end{lstlisting}

\begin{lstlisting}[language=move,caption={Specification of \specurl{bank}{deposit-assets-transfer} in MSL}]
spec bank_addr::bank {
  use std::features;

  spec deposit {
    let addr_sender = signer::address_of(sender);
    let sender_coins_value = global<coin::CoinStore<AptosCoin>>(addr_sender).coin.value;
    let post sender_coins_value_post = global<coin::CoinStore<AptosCoin>>(addr_sender).coin.value;
    let bank_credits = global<Bank>(owner).credits;
    let post bank_credits_post = global<Bank>(owner).credits;
    let bank_credits_sender_coin_value =
    if (simple_map::spec_contains_key(bank_credits, addr_sender))
      { simple_map::spec_get(bank_credits,signer::address_of(sender)).value }
    else
      { 0 };
    let post bank_credits_sender_coin_value_post =  simple_map::spec_get(bank_credits_post,signer::address_of(sender)).value;
    ensures bank_credits_sender_coin_value_post == bank_credits_sender_coin_value + amount;
    requires !features::spec_is_enabled(features::COIN_TO_FUNGIBLE_ASSET_MIGRATION);
    ensures sender_coins_value_post == (sender_coins_value - amount);
  }
}
\end{lstlisting}


\subsection{Multiple-transition invariants}

\subsection{Metamorphic properties}

\begin{figure}[t]
\small
\begin{lstlisting}[language=cvl,caption={Simplified CVL code for the Bank verification},label={fig:specSol}]
// a transaction deposit(amount) aborts if amount is greater than 
// the transaction sender's T balance.  
rule deposit_revert {
    env e;
    require( e.msg.value > nativeBalances[e.msg.sender] );
    deposit@withrevert(e);
    assert lastReverted;
}
\end{lstlisting}
\end{figure}

\begin{figure}[t]
%\small
\begin{lstlisting}[language=move,caption={Simplified MSL code for the Bank verification},label={fig:specMove}]
spec bank_addr::bank {
  spec deposit {
     // the abort condition is an "if", not an "if and only if"
   pragma aborts_if_is_partial = true;
   let sender_coins_val =global<CoinStore>(address_of(sender)).coin.value;
   let bank = global<Bank>(owner); //SERVE?? e' cosi' anche in github
   aborts_if ( sender_coins_val < amount );
   }
}
\end{lstlisting}
\end{figure}


==> rimasugli.tex <==

---------------------------
\section{Rimasugli da cui pescare ancora}
Smart contracts.% e importanza verifica.

\subsection{Traccia di Intro alternativa}

Solidity linguaggio più usato, ma problemi di vario tipo. 

Move linguaggio più recente, più solido (usato Aptos, Sui, IOTA). 
\url{https://github.com/MystenLabs/awesome-move?tab=readme-ov-file}
\enriconote{Dire qui che d'ora in poi con Move ci riferiamo ad Aptos Move}


Nel reame smart contracts, 
la verifica \`e imporante, soprattutto per scongiurare vulnerabilità a livello di business-logic, che sono quelle sui quali gli attacchi reali hanno più impatto~\cite{Chaliasos24icse}.\enriconote{magari citare anche \cite{Xu24langsec}}
\enriconote{attenti a dire questo, perché poi la conclusione potrebbe essere che il Move Prover fa schifo (di proprietà più business-logic ne riesce a verificare ben poche)}
\bartnote{in realtà si potrebbe dire che in Move queste proprietà emergono dalle proprietà delle singole funzioni}
%
Note che esistono molti tool di bug detection, soprattutto per Solidity, ma questi non sono sufficienti per rilevare errori nella business logic.

Specificità dei linguaggi impattano molto sulla possibilità di fare verifica.

In questo articolo siamo interessati a studiare l'impatto che hanno i linguaggi Solidity e Move sulla possibilità di verificare contratti.
\bartnote{se siamo i primi a fare questo (come credo), dirlo esplicitamente}

La capacità di verificare contratti dipende non solo dal linguaggio ma anche, ovviamente, dai tool esistenti.
Per Solidity ricco ecosistema di tool. 
Per Move, Move Prover. 

Come tool prendiamo in considerazione Certora, che riteniamo nel complesso il più espressivo per verifica in Solidity, con Move  il Prover di Aptos (unico mantenuto \enriconote{diciamolo in maniera meno triste}). Specifichiamo che quando determinate proprietà non sono verificabili da Certora ma lo sono da altri tool lo annoteremo espressamente (pur non includendo direttamente questi tool nel confronto).

Prendiamo in considerazione 3 use case rappresentativi.
Per ciascuno use case consideriamo un ampio ventaglio di proprietà: da proprietà più low-level a proprietà di business logic più complesse (tra cui anche trace properties e hyperproperties).

Per ogni proprietà studiamo sia la ground truth (che può dipendere dalle specificità del linguaggio), sia la possibilità di esprimerla e verificarle dai prover (che dipende non solo dal linguaggio ma anche dalle feature dei tool).

Ci interessiamo in particolar modo a quelle che sono le differenze. 

Quali differenze nei linguaggi inducono differenze nella ground truth?

Quali differenze nei linguaggi rendono il compito di verifica diverso? (es.: a volte la verifica è triviale perché implicata dal linguaggio stesso)

Riguardo ai tool: quali funzionalità mancano in uno (o entrambi) necessarie a verificare proprietà interessanti?



%\enriconote{Qualcosa sul confronto}
\bartnote{dire almeno come organizziamo il confronto? Forse anticipare qui i risultati del confronto non si capirebbe}


\ \\

\enriconote{Esistono tool di verifica per altri linguaggi oltre a Solidity e Move? 
 \ 
Certora funziona anche per Vyper (che però compila sempre in EVM bytecode).
 \ 
Per Fe-lang sembra ci sia il progetto di supportare verifica formale, ma ancora tutto demo.
\ 
Rust? Esistono tool di verifica formale per Rust; sono usabili anche nel contesto di smart contracts?
\ 
Tezos: \url{https://opentezos.com/formal-verification/modeling-theorem/}
\
\url{https://github.com/johnsonstephan/awesome-web3-formal-verification} 
Scilla~\cite{Sergey19pacmpl}
}
\enriconote{Questa parte su tool di verifica per altri linguaggio potremmo metterla nei Future work?}

\mypar{Contributions}
We summarise our main contributions as follows.
 \bartnote{meglio presentarlo come summary dei contributi}

\ \\
Struttura:
\begin{itemize}
    \item Introduction 
    \\ + Research Questions?   \enriconote{dove può andare \emph{Research questions}? Al posto del paragrafo \emph{Contributions} nell'Intro?}
    \\ Focusing on Solidity and Move: 
    \begin{enumerate}
        \item How differences in the two languages affect verificability (which properties are impossible to verify, which are trivial, ...).
        \item What is the state-of-the-art of verification tools for Solidity and Move? What can they verify and what not?
        \item (contributions) dataset (nota: è bello averlo anche come supporto per chi impara)
        \\
        \enriconote{un contributo implicito è anche che facciamo la differenza tra 1. e 2.}
    \end{enumerate}
    \item Background (\ref{sec:background}): presentiamo Solidity %(\ref{sec:background:solidity}) 
    e Move %(\ref{sec:background:move})
    e lo stato dell'arte per la loro verifica, e delineiamo differenze tra i due linguaggi (\ref{sec:background:comparison}) \enriconote{\emph{Releted work} è implicitamente qua dentro?}
    \item Methodology (\ref{sec:methodology}): giustifichiamo la scelta dei provers (\ref{sec:methodology:provers}), degli use cases (\ref{sec:methodology:contracts}), e delle proprietà (\ref{sec:methodology:props}).  Accenni su come basare il confronto (questo si sovrapporrà un po' alla sezione Comparison). \enriconote{Forse sottosez \emph{Provers} dopo le altre 2?}
    \item Use cases description (\ref{sec:benchmark}): Breve descrizione degli use cases e di alcune delle proprietà interessanti 
    \item Comparison / Results / Findings (\ref{sec:comparison}): Presentiamo le differenze che abbiamo trovato nella verifica delle specifiche dei 3 use cases. 
    
    In particolare, dividiamo tra differenze che dipendono dal linguaggio (\ref{sec:comparison:language}), e differenze che dipendono dal prover (\ref{sec:comparison:prover}). \enriconote{Secondo me è importante fare questa distinzione a monte: i risultati della prima sottosezione sono di carattere generale e sopravvivranno alla prova del tempo, mentre quelli della seconda possono essere molto utili a chi sviluppa tool di verifica, però comunque dipendono molto dal futuro dei 2 tool considerati e sono più che altro una "fotografia" dello stato dell'arte nel momento della stesura dell'articolo } 
    \item Conclusions / Limitations / Future work (\ref{sec:conclusions}): 
\end{itemize}

%un altro obiettivo è capire quali tipi di proprietà sono esprimibili nei due tool, e quali non lo sono


\subsection{Comparison between Solidity and Move}
\label{sec:background:comparison}
\enriconote{Aggiungere letteratura}

\begin{itemize}

\item Solidity stateful, Move stateless

\item Importante: in Solidity le risorse vanno implementate e gestite correttamente: bug nell'implementazione potrebbero rendere inconsistente l'uso delle risorse (e.g. token implementati male, citare esempi). Esempio concreto: i credits nel bank.
In Move le risorse sono first-order citizens (paradigma di Move \emph{resource-oriented programming}), quindi il linguaggio, e in particolare il sistema di tipi, garantisce che queste vengano usate nel modo corretto. Questo non implica però che non ci possano essere bug nella business logic.

\item Solidity ha dynamic dispatching, Move no

\item Solidity ha il gas che incasina la semantica, Move non lo so (controllare) ???

\item Altro?
\end{itemize}

\subsection{Altre sparse}

SoK su metodi formali per smart contracts: \cite{Tolmach22csur}
\bartnote{da citare, ma come SoK la trovo poco utile}

%Metamorphic testing: \cite{Chen18csur}

How to specify it~\cite{Hughes19tfp} \bartnote{nel titolo dice ``for pure functions'', ma alcuni tipi di proprietà hanno senso anche per programmi stateful}



%\subsection*{RIMASUGLI: Solidity and its verification} 
%\label{sec:background:solidity}


%Esempio snippet di Certora-rule?
%Spiegazione delle rule di Certora, assert/satisfy ecc.



% The Ethereum ecosystem includes several bug detection tools that can spot \emph{specific} forms of liquidity vulnerabilities in smart contracts.
% In that setting, these vulnerabilities are often referred to as ``Locked Ether'', which are roughly described as the absence of a mechanism to withdraw Ether from the contract.
% The tools capable of detecting Locked Ether bugs include   
% Slither~\cite{slither},
% SmartCheck~\cite{smartcheck},
% Maian~\cite{maian},
% Securify2~\cite{Tsankov18ccs},
% ConFuzzius~\cite{confuzzius}
% and sFuzz~\cite{sfuzz}.
% Each of these tools has its own internal encoding of the Locked Ether property, making it difficult to compare them~\cite{Sendner24sp}.
% There are two main differences between these tools and ours.
% First, while these tools can only spot that a predefined hard-coded Locked Ether property is violated, Solvent can verify custom liquidity properties, defined by our specification language.  In particular, Solvent can verify properties that express \emph{who} can withdraw \emph{how much}, and under \emph{which conditions}; not just that Ether does not get frozen in the contract.
% Second, bug detection tools only focus on property violations, while Solvent (a formal verification tool) is capable of verifying that a liquidity property is satisfied (always, or up to a certain bound on the number of transactions).

% Other state-of-the-art formal verification tools for Solidity do not support general liquidity properties.
% SolCMC, the prover shipped with the Solidity compiler, as well as other verification tools such as Zeus~\cite{Kalra18ndss}, solc-verify~\cite{Hajdu19vstte}, VerX~\cite{Permenev20sp} and SmartACE~\cite{Wesley22vmcai}, only support safety properties, while other tools, such as Certora~\cite{certora}, VeriSolid~\cite{Nelaturu23tdsc}, and SmartPulse~\cite{Stephens21sp}, can also verify liveness properties.
% However, this is not enough for liquidity properties.

Quantitative properties~\cite{Chatterjee18esop}??


%\subsection*{RIMASUGLI:Move and its verification}
%\label{sec:background:move}


Citazioni ad articoli che riguardano il Move Prover. \cite{Zhong20cav,Dill22tacas,Xu24langsec}  

Citazioni ad articoli che riguardano il Move Prover di Aptos \cite{Park24fmbc} \cite{AptosCoin}

%Presentazione tipi di spec del Move Prover: unit spec, struct invariant, state invariant, update invariant. 

%Snippet di alcune (tutte?) spec del Move Prover.
%\enriconote{Magari riportare contratto Bank per entrambi e 1 prop per ciascuno (una semplice che non necessita assumptions)}

%\enriconote{Per i vari snippet usiamo uno dei nostri use case? Quale?}

\url{https://aptos.dev/en/build/smart-contracts/move-security-guidelines}


==> taxonomy.tex <==
\section{Taxonomy}

\begin{table}
\begin{tabular}{|c|c|c|c|}
 \hline
 \textbf{Type (primary)} & \textbf{Type (secondary)} &  \textbf{Certora features} & \textbf{Move Prover features } \\ \hline
    \multirow{2}{*}{ \makecell{ Function spec } }
        & success condition & \makecell{rule \\ (require / call / assert @withrevert)} & aborts if + requires \\\cline{2-4}
        & \makecell{postcondition \\ (partial correctness)} & \makecell{rule \\ (require / call / assert)}  & ensures \\
        \hline
    \multirow{2}{*}{ \makecell{ State invariant } }
        & Local & \makecell{invariant} & ? \\\cline{2-4}
        & \makecell{Global} & \makecell{rule}  & \makecell{ struct invariant \\ OR global invariant} \\
        \hline
    \multirow{3}{*}{ \makecell{ Linear properties } }
        & \makecell{Single-transition  \\ invariant} & \makecell{rule (require / assert)} & \makecell{global invariant update \\ OR schema + function specs} \\\cline{2-4}
        & \makecell{Multiple-transition  \\ invariant} & \makecell{rule (require / assert)} & \makecell{\emph{ND}} \\\cline{2-4}
        & \makecell{Liveness} & \makecell{\emph{ND}} & \makecell{\emph{ND}} \\
        \hline
    \multirow{3}{*}{ \makecell{ Branching properties } }
        & \makecell{Metamorphic properties } & \makecell{storage types} & \makecell{\emph{ND}} \\\cline{2-4}
        & \makecell{Enabledness $AG(EX)^*$} & \makecell{\emph{ND}} & \makecell{\emph{ND}} \\\cline{2-4}
        & \makecell{...} & \makecell{} & \makecell{} \\
        \hline
\end{tabular}
\end{table}
